Paths and Intersections: Characterization of Quasi-metrics in Directed Okamura-Seymour Instances

We study the following distance realization problem. Given a quasi-metric $D$ on a set $T$ of terminals, does there exist a directed Okamura-Seymour graph that realizes $D$ as the (directed) shortest-path distance metric on $T$? We show that, if we are further given the circular ordering of terminals lying on the boundary, then Monge property is a sufficient and necessary condition. This generalizes previous results for undirected Okamura-Seymour instances. With the circular ordering, we give a greedy algorithm for constructing a directed Okamura-Seymour instance that realizes the input quasi-metric. The algorithm takes the dual perspective concerning flows and routings, and is based on a new way of analyzing graph structures, by viewing graphs as \emph{paths and their intersections}. We believe this new understanding is of independent interest and will prove useful in other problems in graph theory and graph algorithms. We also design an efficient algorithm for finding such a circular ordering that makes $D$ satisfy Monge property, if one exists. Combined with our result above, this gives an efficient algorithm for the distance realization problem.

==> headers.tex <==
\iffalse
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{patterns}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{snakes}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{petri,decorations.markings}
\fi

\renewcommand{\top}{T}

\RequirePackage{silence}
\WarningFilter{remreset}{The remreset package}
\usepackage{fancybox}
\usepackage{enumitem}

\setlistdepth{9}

\newlist{myEnumerate}{enumerate}{5}
\setlist[myEnumerate,1]{label=\arabic*.}
\setlist[myEnumerate,2]{label=(\alph*)}
\setlist[myEnumerate,3]{label=\roman*.}
\setlist[myEnumerate,4]{label=\Alph*.}
\setlist[myEnumerate,5]{label=\Roman*.}
%\setlist[myEnumerate,6]{label=(\arabic*)}
%\setlist[myEnumerate,7]{label=(\Roman*)}
%\setlist[myEnumerate,8]{label=(\Alph*)}
%\setlist[myEnumerate,9]{label=(\roman*)}

%\usepackage{kbordermatrix}
%\renewcommand{\kbldelim}{(}% Left delimiter
%\renewcommand{\kbrdelim}{)}% Right delimiter
\usepackage{blkarray}
\usepackage{array}
%\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\mLabel}[1]{\mbox{$\scriptstyle{#1}$}}

\usepackage{stackengine}
\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}
%\usepackage{enumerate}

\newcommand{\gy}{G_{\sigma_n}^{\mathrm{yes}}}
\newcommand{\gn}{G_{\sigma_n}^{\mathrm{no}}}
\newcommand{\dtv}{D_{\mathrm{TV}}}

\usepackage{amsmath,amsfonts,amssymb,amsthm,bm}
\usepackage{color,xcolor}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{nameref}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{myred}{rgb}{0.8,0.25,0.25}
\definecolor{DarkRed}{rgb}{0.7, 0.0, 0.0}
\usepackage[linktocpage=true, pagebackref=true,colorlinks, linkcolor=DarkRed,citecolor=ForestGreen, bookmarks,bookmarksopen,bookmarksnumbered]{hyperref}

\usepackage[noabbrev,nameinlink]{cleveref}
\crefname{property}{property}{Property}
\creflabelformat{property}{(#1)#2#3}
\crefname{equation}{eq}{Eq}
\creflabelformat{equation}{(#1)#2#3}
\usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{amsfonts}
\usepackage{thm-restate}
\usepackage{blindtext}
\usepackage{thm-restate}

\iffalse
\textheight 8.5in
\topmargin -0.2in
\oddsidemargin 0.20in
\textwidth 6.3in
\fi

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemm}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{warning}[theorem]{Warning}

\theoremstyle{definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[lemm]{Assumption}
\newtheorem{definition}[lemm]{Definition}
\newtheorem{remark}[lemm]{Remark}
\newtheorem{problem}{Problem}


\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}


\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{%\vskip 0.2in
\noindent
%\begin{figure}
  \begin{center}
\begin{fminipage}{1\textwidth}%{6.3in}
}{
\end{fminipage}
\end{center}
%\end{figure}
%\vskip 0.2in
}

%\newenvironment{probbox}[0]{\vskip 0.1in
%%\noindent 
%  \begin{center}
%        \begin{fminipage}{5.7in}
%}{
%\end{fminipage}
%\end{center}
%\vskip 0.1in
%}

% Algorithm2e
\DontPrintSemicolon
\SetKw{KwAnd}{and}
\SetProcNameSty{textsc}
\SetFuncSty{textsc}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\def\dr{\mathrm{d}}

\def\pleq{\preceq} %curlyeq}
\def\pgeq{\succeq} %curlyeq}
\def\pge{\succ}
\def\ple{\prec}
\def\sc{\textsc{SC}}

\newcommand\AGM{\textsc{UnweightedCutSparsify}}
\newcommand\WGM{\textsc{WeightedCutSparsify}}
\newcommand\WL{\textsc{WeightedEdgeSampler}}

\newcommand\HVS{\textsc{HeavyEdgeSketch}}
\newcommand\HVR{\textsc{HeavyEdgeRecovery}}

\newcommand\WSS{\textsc{SpectralSketch}}
\newcommand\WSR{\textsc{SpectralRecovery}}

\newcommand\SQS{\textsc{SquareSketch}}
\newcommand\SQR{\textsc{SquareRecovery}}

\newcommand\SVS{\textsc{SquareHeavySketch}}
\newcommand\SVR{\textsc{SquareHeavyRecovery}}

\newcommand\SSQ{S^{\mathrm{sq}}}
\newcommand\SSS{S^{\mathrm{ss}}}
\newcommand\SHV{S^{\mathrm{hv}}}
\newcommand\SSV{S^{\mathrm{sqh}}}

\def\detp{\det\nolimits_{+}}
\def\detb#1{\det\nolimits_{#1}}
\def\detz{\det\nolimits_{(0,\zeta]}}
\def\detzz{\det\nolimits_{(0,\zeta']}}
\def\detl{\det\nolimits_{\ell}}
\def\detll{\det\nolimits_{\ell'}}
\def\detn{\det\nolimits}

\def\dr{\mathrm{d}}

\def\Approx#1{\approx_{#1}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}


\def\prob#1#2{\mathrm{Pr}_{#1}\left[ #2 \right]}
\def\pr#1{\mathrm{Pr}\left[ #1 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\mathbb{E}}_{#1}\left[ #2 \right]}
\def\ex#1{{\mathbb{E}}\left[ #1 \right]}
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}
\def\card#1{\left| #1 \right|}
\def\deg{\textrm{deg}}




\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\eps{\epsilon}

\def\abs#1{\left|#1  \right|}

\def\rank#1{\mathrm{rank} \left(#1 \right)}
\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\norm#1{\left\| #1 \right\|}
\def\normm#1{\lambdamax\kh{#1}}
\def\smallnorm#1{\| #1 \|}

\def\comp#1{#1^\complement}

\def\Acal{\mathcal{A}}
\def\Ncal{\mathcal{N}}
\def\Rcal{\mathcal{R}}
\def\Bcal{\mathcal{B}}
\def\Ccal{\mathcal{C}}
\def\Dcal{\mathcal{D}}
\def\Ecal{\mathcal{E}}
\def\Fcal{\mathcal{F}}
\def\Mcal{\mathcal{M}}
\def\Xcal{\mathcal{X}}
\def\Ftil{\tilde{F}}
\def\Htil{\tilde{H}}
\def\Ztil{\tilde{Z}}
\def\Ltil{\tilde{L}}
\def\wtil{\tilde{w}}
\def\Fcaltil{\tilde{\mathcal{F}}}
\def\Lambdatil{\tilde{\Lambda}}
\def\Hcal{\mathcal{H}}
\def\Ical{\mathcal{I}}
\def\Itil{\tilde{{I}}}
\def\Gcal{\mathcal{G}}
\def\Rcal{\mathcal{R}}
\def\phitil{\tilde{\phi}}
\def\Ucal{\mathcal{U}}
\def\Vcal{\mathcal{V}}
\def\Lcal{\mathcal{L}}
\def\Scal{\mathcal{S}}
\newcommand\Tcal{\mathcal{T}}
%\newcommand\Ucal{\mathcal{U}}
\newcommand\Pcal{\mathcal{P}}

\newcommand\xtil{\tilde{x}}
\newcommand\Gtil{\tilde{G}}

\newcommand\pth{\mathfrak{p}}


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

%\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\ppi{\vec{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}

\newcommand\er{R_{\mathrm{eff}}}
\newcommand\ccc{C_{\mathrm{CC}}}
\newcommand\ci{C_{\mathrm{I}}}


\def\lev{\mathtt{lev}}
\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
%\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
%\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
%\renewcommand\ll{\boldsymbol{\mathit{\ell}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand{\ttau}{{\boldsymbol{\mathit{\tau}}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
%\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\nn{\vec{n}}
\newcommand\mm{\vec{m}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\newcommand\rrh{{\boldsymbol{\widehat{\mathit{{r}}}}}}
\renewcommand\dh{\widehat{d}}
\newcommand\wh{\widehat{w}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}

\newcommand\dbar{d_{\mathrm{avg}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\mathrm{\textsf{M}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\HH{\boldsymbol{\mathit{H}}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\TT{\boldsymbol{\mathit{T}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}

\def\sfy{{\sf Yes} }
\def\sfn{{\sf No} }
\newcommand\nnz{\mathrm{nnz}}
\newcommand\tv{\mathrm{TV}}
\newcommand\yes{\mathrm{yes}} % {\mathrm{yes}}
\newcommand\no{\mathrm{no}}

\newcommand\shat{\hat{s}}
\newcommand\ftil{\tilde{f}}
\newcommand\lambdatil{\tilde{\lambda}}
\newcommand\Ntil{\tilde{N}}
\newcommand\dtil{\tilde{d}}
\newcommand\Dtil{\tilde{D}}
\newcommand\MMtil{\boldsymbol{\mathit{\tilde{M}}}}
\newcommand\AAtilde{\boldsymbol{\mathit{\tilde{A}}}}
\newcommand\LLtil{\boldsymbol{\mathit{\tilde{L}}}}
\newcommand\MMtilde{\boldsymbol{\mathit{\tilde{M}}}}

\newcommand\AAn{\boldsymbol{\mathcal{A}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}

\newcommand\ZZtil{\widetilde{\boldsymbol{\mathit{Z}}}}

\newcommand\AAhat{\boldsymbol{\widehat{\mathit{A}}}}
\newcommand\AAapprox{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDhat{\boldsymbol{\widehat{\mathit{D}}}}
\newcommand\DDapprox{\boldsymbol{\widetilde{\mathit{D}}}}
\newcommand\LLhat{\boldsymbol{\widehat{\mathit{L}}}}
\newcommand\LLapprox{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\MMhat{\boldsymbol{\widehat{\mathit{M}}}}
\newcommand\MMapprox{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\ZZhat{\boldsymbol{\widehat{\mathit{Z}}}}

\newcommand\AAtil{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDtil{\boldsymbol{\widetilde{\mathit{D}}}}


\newcommand\bbtil{\boldsymbol{\tilde{\mathit{b}}}}
\newcommand\xxtil{\boldsymbol{\tilde{\mathit{x}}}}


\newcommand\Otil{\tilde{O}}
\newcommand\otil{\tilde{o}}
\newcommand\Ktil{\tilde{K}}
\newcommand\Thetatil{\tilde{\Theta}}
\newcommand\Omegatil{\tilde{\Omega}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\fbf{\mathbf{f}}

\newcommand\Ghat{{\widehat{{G}}}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\diag}{\textsc{diag}}
\newcommand\LLs{\boldsymbol{\mathit{L}_s}}
\newcommand\SSi{\boldsymbol{\Sigma}}

\newcommand\dila{\mathtt{dila}}
\newcommand\cont{\mathtt{ctrc}}
\newcommand\area{\mathtt{area}}
\newcommand\vol{\mathsf{cost}}
\newcommand\scolon{\hspace{-2.5pt}:\hspace{-1.5pt}}

\newcommand\DS{\textsc{DetScheduling}}
\newcommand\DP{\textsc{DPScheduling}}
\newcommand\RI{\textsc{Rounded}}
\newcommand\PTAS{\textsc{PoiScheduling}}
\newcommand\ILP{\textsc{ILPScheduling}}
\newcommand\IP{\textsc{ILP}}
\newcommand\CHEBY{\textsc{ChebySolve}}
\newcommand\HARGD{\textsc{AlmostRegularDecomp}}
\newcommand\HED{\textsc{ExpanderDecomp}}
\newcommand\WAM{\textsc{Whack-a-mole-I}}
\newcommand\WTM{\textsc{Whack-a-mole-II}}
\newcommand\WAME{\textsc{Whack-a-mole-Exp}}

\newcommand\la{\leftarrow}

\newcommand\TEST{\textsc{Traps?}}
\newcommand\MBSWB{\textsc{NoisyBinarySearchRW}}

\newcommand\IR{\textsc{Sparisfy}}
\newcommand\SP{\textsc{SampleWR}}

\newcommand\SC{\mathrm{SC}}
\newcommand\SCN{\mathrm{SC}_n}

\newcommand{\sd}{\geq_{\mathrm{sd}}}

\newcommand{\todo}[1]{{\bf \color{red} TODO: #1}}
\newcommand{\hl}[1]{{\bf \color{orange} Huan: #1}}
%\newcommand{\yhy}[1]{{\color{blue} #1}}
%\newcommand{\zzz}[1]{{\bf \color{green} Zhongzhi: #1}}
%\newcommand{\sep}[1]{{\color{blue}#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\poi}[1]{\mathrm{Poi}\left(#1\right)}

\newcommand{\kh}[1]{\left(#1\right)}

\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}

\newcommand{\wmax}{w_{\max}}
\newcommand{\wmin}{w_{\min}}

\newcommand{\lambdamin}{\lambda_{\mathrm{min}}}
\newcommand{\lambdamax}{\lambda_{\mathrm{max}}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\ade}[1]{{\color{blue}#1}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\dmin}{d_{\mathrm{min}}}


==> intuition.tex <==

Let $T=\set{a,b,t_1,t_2,\ldots,t_{k-2}}$.
Assume that we have already received terminal pairs $(t_1,t_2),(t_3,t_4)$, and we have inserted the paths $\pi_{t_1,t_2},\pi_{t_3,t_4}$ as shown in \Cref{fig: routing1}.
Upon receiving the terminal pair $(a,b)$, there is an $(a,b)$-restricting pair $\cset,\cset'$, where 
\begin{itemize}
	\item $\cset=\set{(a,b),(t_1,t_2),(t_3,t_4)}$; and
	\item $\cset'=\set{(a,t_4),(t_1,b),(t_3,t_2)}$.
\end{itemize}
(Note that this can be easily achieved, for example, by setting $D(a,t_4)=D(t_1,b)=D(t_3,t_2)=3$ and all other distances to be $2$, not violating any directed Monge property.)

Now if we insert the path $\pi_{a,b}$ in the way shown in \Cref{fig: routing2}, then we are in trouble, as there is indeed a routing of $\cset'$ in the resulting nest, shown in \Cref{fig: routing3}, contradicting the requirement in \Cref{clm: demand}. In other words, from the definition of a restricting pair,
\[D(a,b)+D(t_1,t_2)+D(t_3,t_4)<D(a,t_4)+D(t_1,b)+D(t_3,t_2);\]
however, the existence of a $\cset'$-routing means that we can ``extract'' a $t_1$-$b$ path, a $a$-$t_4$ path, and a $t_3$-$t_2$ path, by non-repetitively using the edges from the shortest paths $\pi_{t_1,t_2},\pi_{t_3,t_4}$, and $\pi_{a,b}$, which implies that 
\[D(a,b)+D(t_1,t_2)+D(t_3,t_4)\ge D(a,t_4)+D(t_1,b)+D(t_3,t_2),\]
a contradiction. Therefore, the \Cref{fig: routing2}-way of inserting the path $\pi_{a,b}$ is forbidden. In fact, we can show that the path $\pi_{a,b}$ is not allowed to touch the blue area shown in \Cref{fig: routing1}. This area can be understood as the ``forbidden area'' caused by the restricting pair $(\cset,\cset')$.

\begin{figure}[h!]
	\centering
	\subfigure[Paths $\pi_{t_1,t_2}$ and $\pi_{t_3,t_4}$.]
	{\scalebox{0.08}{\includegraphics{fig/routing1}}\label{fig: routing1}}
	\hspace{0.5cm}
	\subfigure[A way of inserting $\pi_{a,b}$.]
	{
		\scalebox{0.08}{\includegraphics{fig/routing2}}\label{fig: routing2}}
	\hspace{0.5cm}
	\subfigure[The routing of $\cset'$.]
	{
		\scalebox{0.08}{\includegraphics{fig/routing3}}\label{fig: routing3}}
	\caption{An illustration of the restriction caused by the $(a,b)$-restricting pair $(\cset,\cset')$.\label{fig: routing}}
\end{figure}

\subsubsection*{Getting around the forbidden areas}

Our goal is to show that there exists a way of inserting the path $\pi_{a,b}$ that gets around all forbidden areas. Equivalently, we need to show that the union of all forbidden areas does not block the way from $a$ to $b$ inside the disc. 
Note that the disc boundary is separated by $a,b$ into two segments: the left segment (from $b$ clockwise to $a$) and the right segment (from $a$ clockwise to $b$).
Typically, a forbidden area rises from either the left segment or the right segment and extends to somewhere in the middle. Therefore, in an intuitive ``geometry duality'' sense,
\emph{the forbidden areas do not block the $a$-$b$ connection iff there do not exist a forbidden area from the left segment and a forbidden area from the right segment that intersect each other}.

But how can we ensure that there are no such intersecting forbidden areas? As an example, how do we rule out the possibility shown in \Cref{fig: forbidden}, where a forbidden area $p$-$t_1$-$t_4$ from the left segment intersects the forbidden area $q$-$t_6$-$t_7$ from the right segment?

\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.12]{fig/forbidden}
	\caption{An illustration of intersecting forbidden areas (yellow is partially covered by blue).\label{fig: forbidden}}
\end{figure}

The answer is to use the Monge property of the input metric $D$ (this is the first and the only time we use it). Specifically, the forbidden area $p$-$t_1$-$t_4$ is caused by the restricting pair 
\begin{itemize}
	\item $\cset_1=\set{(a,b),(t_1,t_2),(t_3,t_4)}$; and
	\item $\cset'_1=\set{(a,t_4),(t_1,b),(t_3,t_2)}$;
\end{itemize}
and the forbidden area  $q$-$t_6$-$t_7$ is caused by the restricting pair 
\begin{itemize}
	\item $\cset_2=\set{(a,b),(t_5,t_6),(t_7,t_8)}$; and
	\item $\cset'_2=\set{(a,t_6),(t_5,t_8),(t_7,t_b)}$.
\end{itemize}
Therefore, $D(\cset_1)<D(\cset'_1)$ and $D(\cset_2)<D(\cset'_2)$ must hold, so $D(\cset_1)+D(\cset_2)<D(\cset'_1)+D(\cset'_2)$, i.e.,
\begin{equation}
\label{eqn_1}
D\bigg(2(a,b),(t_1,t_2),(t_3,t_4),(t_5,t_6),(t_7,t_8)\bigg)<D\bigg((a,t_4),(t_1,b),(t_3,t_2),(a,t_6),(t_5,t_8),(t_7,t_b)\bigg).
\end{equation}
However, this is impossible, since from the Monge property,
\begin{itemize}
	\item $D(t_1,t_2)+D(t_7,t_8)\ge {\color{red}D(t_1,t_8)}+{\color{blue}D(t_7,t_2)}$, as $(t_1,t_2)$ and $(t_7,t_8)$ cross; and
	\item $D(a,b)+D(t_3,t_4)\ge D(a,t_4)+{\color{brown}D(t_3,b)}$, as $(a,b)$ and $(t_3,t_4)$ cross; and
	\item ${\color{brown}D(t_3,b)}+{\color{blue}D(t_7,t_2)}\ge D(t_3,t_2)+D(t_7,b)$, as $(t_3,b)$ and $(t_7,t_2)$ cross; and
	\item $D(a,b)+D(t_5,t_6)\ge D(a,t_6)+{\color{brown}D(t_5,b)}$, as $(a,b)$ and $(t_5,t_6)$ cross; and
	\item ${\color{brown}D(t_5,b)}+{\color{red}D(t_1,t_8)}\ge D(t_1,b)+D(t_5,t_8)$, as $(t_5,b)$ and $(t_1,t_8)$ cross.
\end{itemize}
Combining all these inequalities, we get that 
\[
D\bigg(2(a,b),(t_1,t_2),(t_3,t_4),(t_5,t_6),(t_7,t_8)\bigg)\ge D\bigg((a,t_4),(t_1,b),(t_3,t_2),(a,t_6),(t_5,t_8),(t_7,t_b)\bigg).
\]
a contradiction to Inequality~\ref{eqn_1}.

To summarize, we refute the intersecting forbidden areas in \Cref{fig: forbidden} by showing that their corresponding pairs $(\cset_1,\cset'_1),(\cset_2,\cset'_2)$ cannot both be restricting pairs. In other words, although there are Monge metrics $D$ allowing $(\cset_1,\cset'_1)$ to be a restricting pair, and there are Monge metrics $D$ allowing $(\cset_2,\cset'_2)$ to be a restricting pair, there are no  Monge metrics $D$ allowing both $(\cset_1,\cset'_1)$ and $(\cset_2,\cset'_2)$ to be restricting pairs.

The core in the analysis above is the very first inequality $D(t_1,t_2)+D(t_7,t_8)\ge {\color{red}D(t_1,t_8)}+{\color{blue}D(t_7,t_2)}$, which is also bridge between two collections $\cset_1,\cset_2$: since $(t_1,t_2)$ as a terminal pair in $\cset_1$ and $(t_7,t_8)$ as a terminal pair in $\cset_2$ cross, we are able to put them together on the LHS of a Monge property, and thereby combine $\cset_1,\cset_2$ to eventually show that in $D$ they cannot be respectively smaller than $\cset'_1,\cset'_2$ simultaneously.

==> route.tex <==
\section{Route}
Each requirement is induced from an inequalities, which can seen as given some of the shortest path, together with the shortest path $AB$, these paths cannot route some demands.

Note that only the shortest path of $AB$ is not fixed, some of the demands can be route without $AB$ {\color{red} (traffic control)}. After the routing of some demands and do some rename, the requirements of drawing $AB$ can be formalized as follows: there is several groups of paths, for each group $i$, there is some path $s^i_jt^i_j$, we require that these path together with the shortest path $AB$ cannot route demands $At^i_1$, $s^i_1t^i_2, \dots, s^i_{J_i} B$. In other words, the shortest path of $AB$ cannot satisfies the following: for each group $i$, the shortest path intersect with each path in the group in order.

We first prove some properties. We say a requirement $st$ is forward parallel to $AB$ if the order of these four point on the outer face is $A,B,t,s$.

\begin{proposition}
    Without lose of generality we can assume that there is no demand $s^i_jt^i_{j+1}$ and $AB$ is forward parallel.
\end{proposition}

For any two point in the plain, we say a path seperate two point if the path intersects with any path that connects these two points. We say a series of paths seperate two points $A$ and $B$ in order, if the first path seperate $A$ and $B$, and for any $i^{th}$, the $(i+1)^{th}$ path seperate every point on the $i^{th}$ path and $B$. We prove the following lemma.

\begin{lemma} \label{lem:induction}
    If no matter how we draw the path from $A$ to $B$, there is a requirement is broken, then there is a requirement such that for each group of paths, the paths seperates $A$ and $B$ in order.
\end{lemma}

We first show that assumming \Cref{lem:induction}, if there is no way to draw the shortest path $AB$, there is an inequality that is contridicted to quadruples condition. By \Cref{lem:induction}, if we cannot draw the shortest path $AB$, we have a requirement such that for each group of paths, the paths seperates $A$ and $B$. Suppose for $i^{th}$ group the paths are $s^i_jt^i_j$, then by some rerouting, the inequality can be written as $\sum_i (AB+\sum_j s^i_jt^i_j) < \sum_i (At^i_1+s^i_1t^i_2+\dots+s^i_{J_i}B)$. For each $i$, by guarantee of \Cref{lem:induction}, $s^i_1t^i_1$ seperates $A$ and $B$, then by quadruples condition, we have $AB + s^i_1t^i_1 \ge At^i_1 + s^i_1B$. Again by guarantee of  \Cref{lem:induction}, $s^i_2t^i_2$ seperates $s^i_1$ and $B$, so $s^i_1B+s^i_2t^i_2 \ge s^i_1t^i_2 + s^i_2B$. We can keep using the same argument, until we get $AB+\sum_j s^i_jt^i_j \ge At^i_1+s^i_1t^i_2+\dots+s^i_{J_i}B$, which contradicts the inequality.

In the rest of the section, we prove \Cref{lem:induction}. 

